PhoneLM:an Efficient and Capable Small Language Model Family through Principled Pre-training

The interest in developing small language models (SLM) for on-device deployment is fast growing. However, the existing SLM design hardly considers the device hardware characteristics. Instead, this work presents a simple yet effective principle for SLM design: architecture searching for (near-)optimal runtime efficiency before pre-training. Guided by this principle, we develop PhoneLM SLM family (currently with 0.5B and 1.5B versions), that acheive the state-of-the-art capability-efficiency tradeoff among those with similar parameter size. We fully open-source the code, weights, and training datasets of PhoneLM for reproducibility and transparency, including both base and instructed versions. We also release a finetuned version of PhoneLM capable of accurate Android Intent invocation, and an end-to-end Android demo. All materials are available at https://github.com/UbiquitousLearning/PhoneLM.

==> fig-pretraining-architecture-rope+relu.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}{4cm}
\centering
\includegraphics[width=1\textwidth]{figs/fig-pretraining-architecture-rope.pdf}
\caption{\yrj{TODO}} \label{fig:pretraining-architecture-rope}
\end{minipage}
\begin{minipage}{4cm}
\centering
\includegraphics[width=1\textwidth]{figs/fig-pretraining-architecture-relu.pdf}
\caption{\yrj{TODO}} \label{fig:pretraining-architecture-relu}
\end{minipage}
\end{figure}




% \begin{figure}[H] %这里使用的是强制位置，除非真的放不下，不然就是写在哪里图就放在哪里，不会乱动
% 	\centering  %图片全局居中
% 	% \vspace{-0.35cm} %设置与上面正文的距离
% 	% \subfigtopskip=2pt %设置子图与上面正文或别的内容的距离
% 	% \subfigbottomskip=2pt %设置第二行子图与第一行子图的距离，即下面的头与上面的脚的距离
% 	% \subfigcapskip=-5pt %设置子图与子标题之间的距离
% 	\subfigure[\yrj{TODO}]{
%         \label{fig:pretraining-architecture-rope}
% 		\includegraphics[width=0.45\linewidth]{figs/fig-pretraining-architecture-rope.pdf}}
% 	\quad %默认情况下两个子图之间空的较少，使用这个命令加大宽度
% 	\subfigure[\yrj{TODO}]{
% 		\label{fig:pretraining-architecture-relu}
% 		\includegraphics[width=0.45\linewidth]{figs/fig-pretraining-architecture-relu.pdf}}
% 	  %这里是空了一行，能够实现强制将四张图分成两行两列显示，而不是放不下图了再换行，使用\\也行。
% 	% \subfigure[level=8]{
% 	% 	\label{level.sub.3}
% 	% 	\includegraphics[width=0.32\linewidth]{./figure/level8.png}}
% 	% \quad
% 	% \subfigure[level=7]{
% 	% 	\label{level.sub.4}
% 	% 	\includegraphics[width=0.32\linewidth]{./figure/level7.png}}
% 	\caption{TODO}
% 	\label{level}
% \end{figure}

==> tab-experimental-other.tex <==
\begin{table*}[ht]
    \centering
    \small
    \subfloat[0.5B]{
        \begin{tabular}{l|c|cccc|ccc}
            \hline
            \textbf{name} & \textbf{size} & \textbf{SocialIQA} & \makecell{\textbf{TruthfulQA}\\\textbf{MC1}} & \makecell{\textbf{TruthfulQA}\\\textbf{MC2}} & \makecell{\textbf{TruthfulQA}\\\textbf{zh MC2}} & \textbf{MMLU} & \textbf{CMMLU} & \textbf{C-Eval Valid} \\
            \hline
            Pythia-410M & 410M & 32.9 & 23.7 & 41.2 & 47.9 & 23.6 & 25.3 & 23 \\
            OPT-350M & 350M & 32.9 & 23.3 & 40.8 & 47.3 & 23.1 & 25.4 & 22.5 \\
            BLOOM-560M & 560M & 34.2 & 25 & 42.4 & 41.6 & 23 & 25.3 & 23 \\
            MobiLlama-0.5B & 500B & 32.9 & 23.3 & 37.5 & 42 & 24.9 & 25.3 & 21.6 \\
            OpenELM-450M & 450M & 32.8 & 24.8 & 40.2 & 47.5 & 25.9 & 24.9 & 22.7 \\
            SmolLM-360M & 360M & 32.9 & 24.6 & 37.9 & 47.4 & 25.8 & 25.4 & 25.7 \\
            \hline
            \textcolor{lightgray}{Qwen1.5-0.5B} & \textcolor{lightgray}{500M} & \textcolor{lightgray}{33.3} & \textcolor{lightgray}{23.6} & \textcolor{lightgray}{38.3} & \textcolor{lightgray}{41.3} & \textcolor{lightgray}{36.5} & \textcolor{lightgray}{47.4} & \textcolor{lightgray}{49.9} \\
            % \textcolor{lightgray}{LaMini-GPT-774M} & \textcolor{lightgray}{774M} & \textcolor{lightgray}{32.8} & \textcolor{lightgray}{22.8} & \textcolor{lightgray}{40.3} & \textcolor{lightgray}{48.5} & \textcolor{lightgray}{26.6} & \textcolor{lightgray}{25.3} & \textcolor{lightgray}{23.1} \\
            \textcolor{lightgray}{Cerebras-GPT-590M} & \textcolor{lightgray}{590M} & \textcolor{lightgray}{33.1} & \textcolor{lightgray}{25.1} & \textcolor{lightgray}{44.1} & \textcolor{lightgray}{47.5} & \textcolor{lightgray}{23.1} & \textcolor{lightgray}{25.3} & \textcolor{lightgray}{22.9} \\
            \hline
            \textbf{PhoneLM-0.5B} & \textbf{500M} & \textbf{42.5} & \textbf{21.9} & \textbf{36.5} & \textbf{43} & \textbf{25.4} & \textbf{24.6} & \textbf{23.6} \\
            \hline
        \end{tabular}
        \label{tab:performance-other-0.5B}
    }
    \quad
    \subfloat[1.5B]{
            \begin{tabular}{l|c|cccc|ccc}
            \hline
            \textbf{name} & \textbf{size} & \textbf{SocialIQA} & \makecell{\textbf{TruthfulQA}\\\textbf{MC1}} & \makecell{\textbf{TruthfulQA}\\\textbf{MC2}} & \makecell{\textbf{TruthfulQA}\\\textbf{zh MC2}} & \textbf{MMLU} & \textbf{CMMLU} & \textbf{C-Eval Valid} \\
            \hline
                Pythia-1.4B & 1.4B & 33.6 & 22.8 & 38.9 & 44.9 & 24.4 & 25.3 & 23 \\
                OPT-1.3B & 1.3B & 32.7 & 24.1 & 38.7 & 47 & 25.2 & 25.3 & 23 \\
                BLOOM-1.1B & 1.1B & 33.5 & 25.3 & 41.8 & 40.5 & 24 & 25.4 & 24.1 \\
                TinyLlama-1.1B & 1.1B & 32.9 & 22 & 37.3 & 42.6 & 24.9 & 24.7 & 24.2 \\
                MobileLLaMA-1.4B & 1.4B & 33 & 21.7 & 34.8 & 43.5 & 24.5 & 25.2 & 23.1 \\
                MobiLlama-1B & 1.0B & 32.9 & 21.7 & 35.2 & 41.6 & 25.4 & 25.4 & 25.3 \\
                OpenELM-1.1B & 1.1B & 32.7 & 22.2 & 37 & 47.3 & 25.3 & 25.3 & 23.4 \\
                DCLM-1B & 1.0B & 44.3 & 22.8 & 36.5 & 43.8 & 46.5 & 30.6 & 29.3 \\
                SmolLM-1.7B & 1.7B & 43.6 & 24.4 & 38.5 & 44.8 & 27.7 & 25.2 & 24.5 \\
                \hline
                \textcolor{lightgray}{Qwen1.5-1.8B} & \textcolor{lightgray}{1.8B} & \textcolor{lightgray}{32.9} & \textcolor{lightgray}{25.8} & \textcolor{lightgray}{39.4} & \textcolor{lightgray}{42.3} & \textcolor{lightgray}{45.4} & \textcolor{lightgray}{59.1} & \textcolor{lightgray}{61.1} \\
                % \textcolor{lightgray}{LaMini-GPT-1.5B} & \textcolor{lightgray}{1.5B} & \textcolor{lightgray}{32.6} & \textcolor{lightgray}{26.2} & \textcolor{lightgray}{42.5} & \textcolor{lightgray}{47.4} & \textcolor{lightgray}{34.6} & \textcolor{lightgray}{25.2} & \textcolor{lightgray}{23.3} \\
                \textcolor{lightgray}{Galactica-1.3B} & \textcolor{lightgray}{1.3B} & \textcolor{lightgray}{32.5} & \textcolor{lightgray}{24.8} & \textcolor{lightgray}{41.4} & \textcolor{lightgray}{47.1} & \textcolor{lightgray}{27.7} & \textcolor{lightgray}{25.2} & \textcolor{lightgray}{22.7} \\
                \textcolor{lightgray}{StableLM2-1.6B} & \textcolor{lightgray}{1.6B} & \textcolor{lightgray}{32.9} & \textcolor{lightgray}{30.6} & \textcolor{lightgray}{45.1} & \textcolor{lightgray}{48.8} & \textcolor{lightgray}{41.1} & \textcolor{lightgray}{30.3} & \textcolor{lightgray}{31.6} \\
                \textcolor{lightgray}{Cerebras-GPT-1.3B} & \textcolor{lightgray}{1.3B} & \textcolor{lightgray}{32.8} & \textcolor{lightgray}{24.5} & \textcolor{lightgray}{42.7} & \textcolor{lightgray}{46.2} & \textcolor{lightgray}{23} & \textcolor{lightgray}{25.3} & \textcolor{lightgray}{23} \\
                \textcolor{lightgray}{MiniCPM-1B} & \textcolor{lightgray}{1.0B} & \textcolor{lightgray}{32.6} & \textcolor{lightgray}{23.1} & \textcolor{lightgray}{36.9} & \textcolor{lightgray}{37.4} & \textcolor{lightgray}{44.9} & \textcolor{lightgray}{47.4} & \textcolor{lightgray}{47} \\
                \textcolor{lightgray}{MiniCPM-2B} & \textcolor{lightgray}{2.0B} & \textcolor{lightgray}{32.9} & \textcolor{lightgray}{25.2} & \textcolor{lightgray}{40.5} & \textcolor{lightgray}{41.8} & \textcolor{lightgray}{45.6} & \textcolor{lightgray}{44.4} & \textcolor{lightgray}{43.2} \\
                \textcolor{lightgray}{Gemma-2B} & \textcolor{lightgray}{2.0B} & \textcolor{lightgray}{33} & \textcolor{lightgray}{22.2} & \textcolor{lightgray}{33.1} & \textcolor{lightgray}{43.6} & \textcolor{lightgray}{32.9} & \textcolor{lightgray}{28.4} & \textcolor{lightgray}{26.1} \\
                \textcolor{lightgray}{Gemma2-2B} & \textcolor{lightgray}{2.0B} & \textcolor{lightgray}{51.2} & \textcolor{lightgray}{24.1} & \textcolor{lightgray}{36.2} & \textcolor{lightgray}{41.3} & \textcolor{lightgray}{49.6} & \textcolor{lightgray}{34.5} & \textcolor{lightgray}{35} \\
                \hline
                \textbf{PhoneLM-1.5B} & \textbf{1.5B} & \textbf{43.2} & \textbf{20.9} & \textbf{33.3} & \textbf{46.1} & \textbf{26.5} & \textbf{25.0} & \textbf{25.7} \\
                \hline
        \end{tabular}
        \label{tab:performance-other-1.5B}
    }
    \caption{Some other Benchmark Score of \llm. \mwx{I suggest we do not show these results.}}
    \label{tab:performance-other}
\end{table*}

==> tab-experimental-sft.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l|l|ccccccc|c}
        \hline
        \textbf{name} & \textbf{type} & \textbf{ARC-e} & \textbf{ARC-c} & \textbf{HellaSwag} & \textbf{WinoGrande} & \textbf{PIQA} & \textbf{SciQ} & \textbf{BoolQ} & \textbf{AVG} \\
        \hline
        \multirow{2}{*}{0.5B} & Base & 60.4 & 31.6 & 54.0 & 57.9 & 73.3 & 85.1 & 60.7 & 60.43 \\
        & SFT & 60.4 & 31.6 & 54.0 & 57.9 & 73.3 & 85.1 & 60.7 & 60.43 \\
        \hline
        \multirow{2}{*}{1.5B} & Base & 66.5 & 39.9 & 65.9 & 61.9 & 75.7 & 88.3 & 66.3 & 66.36 \\
        & SFT & 66.5 & 39.9 & 65.9 & 61.9 & 75.7 & 88.3 & 66.3 & 66.36 \\
        \hline
    \end{tabular}
    \caption{SFT Performance \yrj{TODO:change to other tasks}}
    \label{tab:experimental-sft}
\end{table*}

==> tab-function-calling.tex <==
\begin{table}[ht]
    \centering
    % \small
    % \footnotesize
    \scriptsize
	\subfloat[Stable Training Stage]{
    \begin{tabular}{l|l|r}
        \hline
        \textbf{type} & \textbf{dataset} & \textbf{token} \\
        \hline
        % \qquad\qquad\qquad\qquad 
        web\qquad\qquad\qquad& DCLM-baseline~\cite{li2024datacomplm}\qquad\qquad\qquad & 1.35T \\
        \hline
        code & StarCoderData~\cite{li2023starcoder} & 112.75B \\
        \hline
        \multirow{2}{*}{math} & OpenWebMath~\cite{paster2023openwebmath} & 13.25B \\
        & Dolma-algebraic~\cite{dolma} & 12.75B \\
        \hline
        academic & Dolma-arxiv~\cite{dolma} & 29B \\
        \hline
        \multicolumn{2}{c|}{\textbf{total}} & \textbf{1.5T} \\
        \hline
    \end{tabular}
	\label{tab:pretraining-data-stage1}
    }
	\quad %默认情况下两个子图之间空的较少，使用这个命令加大宽度
	\subfloat[Decay Stage]{
    \begin{tabular}{l|l|r}
        \hline
        \textbf{type} & \textbf{dataset} & \textbf{token} \\
        \hline
        web & DCLM-baseline~\cite{li2024datacomplm} & 10B \\
        \hline
        \multirow{2}{*}{chat} & StarCoderData~\cite{li2023starcoder} & 1.575B \\
         & The Stack Smol & 0.95B \\
        \hline
        \multirow{2}{*}{acadamic}  & Dolma-arxiv~\cite{dolma} & 2.325B \\
         & Dolma-pes2o~\cite{dolma} & 2.35B \\
        \hline
        math instruct & MathInstruct~\cite{yue2023mammoth} & 65.25M \\
        \hline
        \multirow{3}{*}{chat instruct}  & UltraChat~\cite{ding2023enhancing} & 1.775B \\
         & OpenAssistant 2~\cite{kopf2024openassistant} & 42.25M \\
         & OpenHermes~\cite{openhermes} & 77.25M \\
        \hline
        \multirow{4}{*}{code instruct} & Magicoder Evol Instruct~\cite{magicoder} & 30.25M \\
         & CommitPackFT~\cite{muennighoff2023octopack} & 0.35B \\
         & Magicoder OSS Instruct~\cite{MagicoderOSSInstruct75K} & 43.5M \\
         & SlimOrca~\cite{SlimOrca} & 209.75M \\
        \hline
        \multirow{2}{*}{\makecell{function calling\\instruct}} & APIGen~\cite{liu2024apigen} & 48.25M \\
         & Glaive Function Calling~\cite{glaive-function-calling} & 57.5M \\
        \hline
        \multicolumn{2}{c|}{\textbf{total}} & \textbf{20B} \\
        \hline
    \end{tabular}
	\label{tab:pretraining-data-stage2}
    }
	\quad %默认情况下两个子图之间空的较少，使用这个命令加大宽度
    \subfloat[Instruct Turning Stage]{
    \begin{tabular}{l|l|r}
        \hline
        \textbf{type} &\textbf{dataset} & \textbf{token} \\
        \hline
        math instruct & MathInstruct~\cite{yue2023mammoth} & 65.25M \\
        \hline
        \multirow{3}{*}{chat instruct}  & UltraChat~\cite{ding2023enhancing} & 1.775B \\
         & OpenAssistant 2~\cite{kopf2024openassistant} & 42.25M \\
         & OpenHermes~\cite{openhermes} & 77.25M \\
        \hline
        \multirow{4}{*}{code instruct} & Magicoder Evol Instruct~\cite{magicoder} & 30.25M \\
         & CommitPackFT~\cite{muennighoff2023octopack} & 0.35B \\
         & Magicoder OSS Instruct~\cite{MagicoderOSSInstruct75K} & 43.5M \\
         & SlimOrca~\cite{SlimOrca} & 209.75M \\
        \hline
        \multicolumn{2}{c|}{\textbf{total}} & \textbf{2.59B} \\
        \hline
    \end{tabular}
    \label{tab:pretraining-data-sft}
    }
    \caption{The classification of the datasets used in each stage and the number of their tokens. The description of the datasets is in appendix~\ref{sec:appendix-dataset}.}
    \label{tab:pretraining-data}
\end{table}


